TOI-2447 b / NGTS-29 b: a 69-day Saturn around a Solar analogue

Discovering transiting exoplanets with relatively long orbital periods ($>$10 days) is crucial to facilitate the study of cool exoplanet atmospheres ($T_{\rm eq} < 700 K$) and to understand exoplanet formation and inward migration further out than typical transiting exoplanets. In order to discover these longer period transiting exoplanets, long-term photometric and radial velocity campaigns are required. We report the discovery of TOI-2447 b ($=$ NGTS-29b), a Saturn-mass transiting exoplanet orbiting a bright (T=10.0) Solar-type star (T$_{\rm eff}$=5730 K). TOI-2447 b was identified as a transiting exoplanet candidate from a single transit event of 1.3% depth and 7.29 h duration in $TESS$ Sector 31 and a prior transit event from 2017 in NGTS data. Four further transit events were observed with NGTS photometry which revealed an orbital period of P=69.34 days. The transit events establish a radius for TOI-2447 b of $0.865 \pm 0.010\rm R_{\rm J}$, while radial velocity measurements give a mass of $0.386 \pm 0.025 \rm M_{\rm J}$. The equilibrium temperature of the planet is $414$ K, making it much cooler than the majority of $TESS$ planet discoveries. We also detect a transit signal in NGTS data not caused by TOI-2447 b, along with transit timing variations and evidence for a $\sim$150 day signal in radial velocity measurements. It is likely that the system hosts additional planets, but further photometry and radial velocity campaigns will be needed to determine their parameters with confidence. TOI-2447 b/NGTS-29b joins a small but growing population of cool giants that will provide crucial insights into giant planet composition and formation mechanisms.

==> CHRION_pfs_authors.tex <==
\author[0000-0002-8964-8377]{Samuel N. Quinn}
\affiliation{Center for Astrophysics | Harvard \& Smithsonian, 60 Garden St, Cambridge, MA 02138, USA}

\author[0000-0001-6637-5401]{Allyson Bieryla}
\affiliation{Center for Astrophysics | Harvard \& Smithsonian, 60 Garden St, Cambridge, MA 02138, USA}

\author[0000-0001-6588-9574]{Karen A.\ Collins}
\affiliation{Center for Astrophysics | Harvard \& Smithsonian, 60 Garden St, Cambridge, MA 02138, USA}

\author[0000-0002-4297-5506]{Paul A. Dalba}
\affiliation{Department of Astronomy and Astrophysics, University of California, Santa Cruz, CA 95064, USA}
\affiliation{Department of Earth and Planetary Sciences, University of California Riverside, 900 University Avenue, Riverside, CA 92521, USA}

\author[0000-0001-8812-0565]{Joseph E. Rodriguez}
\affiliation{Department of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA}

\author[0000-0002-4891-3517]{George Zhou}
\affiliation{University of Southern Queensland, Centre for Astrophysics, West Street, Toowoomba, QLD 4350 Australia}

\author[0000-0003-1305-3761]{R.P. Butler}
\affiliation{Carnegie Earth and Planets Laboratory, 5241 Broad Branch Road NW, Washington, DC 20015, USA }

\author[0000-0002-5226-787X]{Jeffrey D. Crane}
\affiliation{The Observatories of the Carnegie Institution for Science, 813 Santa Barbara St., Pasadena, CA 91101, USA}

\author{Stephen A. Shectman}
\affiliation{The Observatories of the Carnegie Institution for Science, 813 Santa Barbara St., Pasadena, CA 91101, USA}

\author{Johanna K. Teske}
\affiliation{Carnegie Earth and Planets Laboratory, 5241 Broad Branch Road NW, Washington, DC 20015, USA }

\author{Sharon X. Wang}
\affiliation{Department of Astronomy, Tsinghua University, Beijing 100084, China}

==> planet_c.tex <==
% \section{Orbital solution of a two-planet system}\label{sec:discussion:additional_planets}



% \begin{figure}
%     \centering
%     \includegraphics[width=0.46\textwidth]{TOI-2447_2_planet_fit_lcfit_ttv.pdf}
%     \caption{Orbital solution for \systemb\ and an additional planet. Transit photomety (black) is shown \tess\ (upper panel) and \ngts\ (upper middle panel) with best fitting models (red). Lower panels - radial velocity measurements with best-fitting model (red) for each planet. Semi-transparent error bars represent uncertainties with jitter values added in quadrature.}
%     \label{fig:TOI-2447_b_orbital_2planet}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics{TOI-2447_2_planet_fit_lcfit_2planet_parameter.pdf}
%     \caption{Upper panel: Mass-period diagram of well-characterised transiting exoplanets (mass to better than 50\% precision and radius to better than 20\%; exoplanetarchive.ipac.caltech.edu, accessed 2022-10-07). \systemb\ is indicated in red with the lower bounds of the additional planet marked in green. }
%     \label{fig:TOI-2447_b_additional_planet_MP}
% \end{figure}


% The reflex motion of \systemb\ does not completely explain radial velocity measurements for the \system\ system (Figures \ref{fig:RV_powers} \& \ref{fig:TOI-2447_b_orbital}). The majority of radial velocity measurements come from \harps\ and \chiron, so it follows that these are checked independently for additional planetary signals. The right panels of Figure \ref{fig:RV_powers} reveals that a significant peak at 150 days in the Lomb-Scargle power for \chiron\ data once the reflex motion from planet b is removed. This peak is less convincing in the equivalent \harps\ data where there are significantly fewer observations which have tighter uncertainties. Therefore we state that there is tentative evidence of a third planet in this system with an orbital period near 160 days.

% We performed a 2-planet fit of the \system\ system for \systemb\ and the additional planet candidate with orbital periods of 69 days and 150 days respectively. Our fit included 5 additional parameters to those described in Section \ref{sec:analysis:orbital} corresponding to the additional planet: $\rm T_0$, Period, $K_{\rm 1}$, $f_{\rm s}$, and $f_{\rm c}$. We used an liberal uniform prior between JD 2459347.73941 and 2459387.73941 for the transit epoch, along with a uniform prior between 130 and 170 days for the orbital period. The priors for $K_{\rm 1}$, $f_{\rm s}$, and $f_{\rm c}$ were identical to \systemb\ and we performed identical Bayesian sampling as described in Section \ref{sec:analysis:orbital}. The best-fitting orbital solution shown in Figure \ref{fig:TOI-2447_b_orbital_2planet} and Table \ref{tab:fitted_parameters_2planet} along with derived parameters in Table \ref{tab:derived_parameters_2planet}.

% The two-planet orbital solution does slightly lower the derived mass of \systemb\ but is consistent to within $3-\sigma$ and indicates that the single planet orbital solution may be susceptible to systematic errors due to additional signals in radial velocity measurements. The derived lower-limit for the mass of the additional planet is similar to that of \systemb, although the true value is likely higher given the orbit may be inclined. The significant separation between the orbits of each planet is such that we would not expect significant gravitational interactions. However the orbital periods are close to a 2:1 resonance (ratio = 2.13) where significant transit timing variations maybe be expected where there is a low-order period commensurability \citep[e.g.][]{2018haex.bookE....D}. However, we find that similar 2-planet systems with shorter orbital periods that reside in 2:1 resonances \citep[e.g.][]{2023MNRAS.523.3090T} have no significant transit timing variations and so we expect another body in the system to be the origin of the transit timing variations for \systemb. 

% We checked if the ephemerides of this additional planet is consistent with the unaccounted for transit in \ngts\ observations ($\sim JD =2458145.82$). If the ephemerides and uncertainties for the additional planet in Table~\ref{tab:fitted_parameters_2planet} are propagated back 8 orbital cycles, we estimate an epoch $JD \sim 2458190 + 32 - 35$. This is consistent with the \ngts\ transit to better than 2-$\sigma$ but remains tentative evidence that the two signals are connected. Furthermore, the transit depth from this event cannot be measured although we would expect it to be a similar depth to that of \systemb.

% We inspected the Bayesian information criterion (BIC) for \harps\ and \chiron\ radial velocity observations to find further statistical evidence supporting an additional planet. When comparing the single and two-planet models we found a $\Delta BIC=-283.8$; substantial evidence to favour the 2-planet model over a single planet counterpart. This is the case of both \harps\ ($\Delta BIC=-195.5$) and \chiron ($\Delta BIC=-88.3$). A less rigorous argument can be derived from the radial velocity residuals and the fitted jitter terms in both models. \system\ is a slowly rotating Sun-like star (\vsini $\sim 3.5\,\rm km\, \rm s^{-1}$) and so the expected stellar activity jitter should be low ($\leq 3.5\,\rm m\, \rm s^{-1}$). In the 1-planet fit, a high-precision instrument like \harps\ would be sensitive to the stellar signal but requires an additional jitter value of 5.4$\rm m\, \rm s^{-1}$, suggesting there may be a source of RV scatter beyond the stellar signal. The values decrease in the two-planet fit to 4.3$\rm m\, \rm s^{-1}$ and is more in line with expectations, although not definitive. These arguments are speculative and so we adopt the single planet solution until further observations can be made with regard to the second planet. 

% The evolution and history of planetary systems are encoded in their presently observed orbital solutions. For example, our solar system is broadly consistent with the theory of planet formation in a circumstellar disk \citep[e.g.][]{2009A&A...496..249B} but it is important to understand the architecture of exoplanet systems so that wider and more diverse constraints on planet formation and evolution can be formed. If the outer planet is real, it resides close to the 2:1 mean motion resonance which is possible with convergent disk migration due to disk torques \citep[e.g][]{2002ApJ...567..596L}. This would lead to significant eccentricity excitation which is not supported in our 2-planet model but it remains possible that the planets did not migrate very far or experienced substantial eccentricity dampening. However, the eccentricity of both planets is significantly non-zero and likely that both planets did not form in-situ if parallels are drawn with the similar system, GJ 876 b and c  \citep[orbital periods of 61 days and 30 days respectively][]{2005ApJ...622.1182L}. We do not see any transit signals other than \systemb\ in either \tess\ or \ngts\ data which has coverage in the 1-$\sigma$ transit window predicted in Table \ref{tab:fitted_parameters_2planet}. It is possible that inclination-type resonance capture could excite planet c into a high mutual inclination that is non-transiting although the lack of eccentricity in the inner planet suggests this is unlikely \citep[e.g.][]{2003ApJ...597..566T}. Finally, the architecture of the \system\ system may result in radial velocity measurements that are not accurately described by Keplerian orbits and require Newtonian integration as in the case of GJ 876 \citep[e.g.][]{2001ApJ...551L.109L,2001ApJ...558..392R}. If this is required in the \system-system, it might explain the radial velocity residuals and required jitter values we measure for \harps, \pfs, and \feros. 


% \begin{table}
% \caption{Orbital solution of the \systemb\ and a candidate planet. Asymmetric errors are reported in brackets and correspond to the difference between the median and the 16$^{th}$ (lower value) and 84$^{th}$ (upper value) percentile.}              % title of Table
% \label{tab:fitted_parameters_2planet}      % is used to refer this table in the text
% \centering   
% %                                   % used for centering table
% \begin{tabular}{l c}          % centered columns (4 columns)
% \hline\hline                        % insert
% Parameter & value\\
% \hline 
% \textbf{TOI-2447\,b} \\


% $\rm T_{\rm 0}$ [JD]  & $2458059.61052_{(220)}^{(209)}$  \\
% $\rm T_{\rm 16}$ [JD] & $2459168.98815_{(68)}^{(65)}$  \\
% $\rm T_{\rm 18}$ [JD] & $2459307.68211_{(281)}^{(296)}$  \\
% $\rm T_{\rm 21}$ [JD] & $2459515.68921_{(197)}^{(189)}$  \\
% $\rm T_{\rm 27}$ [JD] & $2459931.70104_{(226)}^{(233)}$  \\
% $R_{\rm 1} / a$  & $0.01559_{(120)}^{(115)}$  \\
% $R_{\rm 2} / R_{\rm 1}$  & $0.08764_{(94)}^{(106)}$  \\
% $b$ & $0.38625_{(16081)}^{(11033)}$  \\
% $zp_{\rm 0}$ & $1.00109_{(15)}^{(15)}$  \\
% $zp_{\rm 16}$ & $1.00000_{(8)}^{(7)}$  \\
% $zp_{\rm 18}$ & $0.99976_{(36)}^{(37)}$  \\
% $zp_{\rm 21}$ & $1.00031_{(16)}^{(16)}$  \\
% $zp_{\rm 27}$ & $0.99966_{(13)}^{(14)}$  \\
% $\rm h_{\rm 1, \ngts}$ & $0.75570_{(270)}^{(274)}$  \\
% $\rm h_{\rm 2, \ngts}$ & $0.73496_{(4354)}^{(4539)}$  \\
% $\rm h_{\rm 1, \tess}$ & $0.78015_{(271)}^{(287)}$  \\
% $\rm h_{\rm 2, \tess}$ & $0.78057_{(4152)}^{(4366)}$  \\
% $K_{\rm 1}$ [m\,s$^{-1}$]  & $14598_{(1535)}^{(1467)}$  \\
% $f_{\rm s}$ & $-0.055_{(170)}^{(225)}$  \\
% $f_{\rm c}$ & $-0.114_{(138)}^{(123)}$  \\ \\

% \textbf{Additional planet} \\
% $\rm T_{\rm 0}$ [JD] & $2459374.07108_{(739029)}^{(957917)}$  \\
% $\rm Period$\,[day] & $148.01625_{(309085)}^{(312078)}$  \\
% $K_{\rm 1}$ [m\,s$^{-1}$]  & $11.621_{(1795)}^{(2142)}$  \\
% $f_{\rm s}$ & $0.265_{(230)}^{(225)}$  \\
% $f_{\rm c}$ & $-0.259_{(389)}^{(315)}$  \\ \\

% \textbf{Common parameters} \\
% $\sigma_{\rm TESS}$ & $0.00023_{(15)}^{(12)}$  \\
% $\sigma_{\rm NGTS}$ & $0.00042_{(8)}^{(8)}$  \\
% $V_0$ \harps\ [km\,s$^{-1}$]  & $3028.44_{(114)}^{(991)}$  \\
% $V_0$ \chiron\ [km\,s$^{-1}$] & $1564.29_{(210)}^{(205)}$  \\
% $J_{\rm HARPS}$ [m\,s$^{-1}$]  & $4.32_{(85)}^{(96)}$  \\
% $J_{\rm CHIRON}$ [m\,s$^{-1}$]  & $12.51_{(197)}^{(206)}$  \\ \\

% \hline
% \end{tabular}
% \end{table}


% \begin{table}
% \caption{Derived and physical properties of the \systemb\ and \systemc\ system. Asymmetric errors are reported in brackets and correspond to the difference between the median and the 16$^{th}$ (lower value) and 84$^{th}$ (upper value) percentile.}              % title of Table
% \label{tab:derived_parameters_2planet}      % is used to refer this table in the text
% \centering   
% %                                   % used for centering table
% \begin{tabular}{l c}          % centered columns (4 columns)
% \hline\hline                        % insert
% Parameter & value\\
% \hline 
% \textbf{TOI-2447\,b} \\
% Period [day] & $69.33683_{(11)}^{(9)}$  \\
% $M_{\rm 2}$ [\mjup] & $0.305_{(26)}^{(37)}$  \\
% $R_{\rm 2}$ [\rjup] & $0.859_{(12)}^{(11)}$  \\
% width [hr] & $8.40_{(84)}^{(11)}$  \\
% $g_{\rm 2}$\,$\rm [m \, \rm s^{-2}]$  & $8.1_{(6)}^{(31)}$  \\
% $e$ & $0.01_{(1)}^{(11)}$  \\
% $\omega$ & $-2.69_{(88)}^{(358)}$  \\
% $\rm T_{\rm eq,b}$ [K] & $465_{(41)}^{(4)}$  \\
% ltt [s] & $149_{(22)}^{(2)}$  \\ \\

% \textbf{TOI-2447\,c} \\
% $M_{2}\sin i$ [\mjup] &  $0.310_{(41)}^{(60)}$ \\
% $e$ & $0.14_{(10)}^{(14)}$\\
% $\omega$ [rad] & $2.34_{(455)}^{(7)}$ \\
% \hline
% \end{tabular}
% \end{table}





% % https://arxiv.org/pdf/2204.08984.pdf
% % In [4]: bruce2.utils.transit_properties.JWST_transmission_metric(1.006, 0.865*c.R_jup.to(c.R_sun).value, 0.386*c.M_jup.to(c.M_sun).value, 420, 9.485)
% % Out[4]: 44.94877333116865
% % This is the fourth quartile from their table 1






==> referee_response_R2_old.tex <==
Dear editor, 

Thank you for sending through the referee report. Below we have addressed the referees concerns.

Regarding the Assistant editors comments, we have reduced the number of keywords down to 6 - my apologies for overlooking that. 

Note: We have added a reference to a recent relevant publication Rodel et al 2024, in addition to Cooke et al 2018 and Villenueva et al 2019 in the introducton

Warm regards, 

Gill et al.



Dear Reviewer,

Thank you for taking the time to look at our paper again. We understand your concerns regarding Section 4.2 and have made substantial effort to improve it. 

Below are detailed comments replying to your report, with our reponse marked with -->.

Warmest regards,

Gill et al. 



Comments to the Author 
This a very interesting discovery, and I commend the authors on their work pursuing this target and writing it up. Most of my concerns have been satisfactorily addressed. However, I think more work is needed before the paper warrants publication. 

I find the discussion of rotation in section 4.2 to be lacking, partly because of the insistence on using the PDCSAP flux: 1) it is risky in general with TESS data (except for young/active stars for which it is more unlikely for the rotation signal to be removed by the PDC pipeline), 2) ~6 days is typical for a false signal induced by PDC (compute the periods of a large number of field stars using PDCSAP light curves and plot a histogram of the results; compare this to what you get using an alternative systematics correction), 3) the relative significance of these signals is not quantified (e.g. by computing false alarm probabilities), and 4) if other methods (lightkurve's regression/PLD) were used as a check on PDC then I would argue those results should be presented either alongside or *instead of* the PDC results, as they are likely to be more reliable, and if they yield the same results (if presented alongside) then at least the reader will be reassured. The reason I previously suggested using these other methods (or even just using SAP flux) was to robustly determine the rotation period, not to check on the transit signal (a point which seems a bit confused in the author response about this). Rotation can be difficult to robustly determine for old/quiet stars. It seems to me that the authors could do a more thorough job in this regard and this could be made more evident to the reader, which would strengthen the result. 


--> We have now added false alarm thresholds for the power spectra presented in section 4.2. 
--> In our previous referee response, we stated "not to check on the transit signal" -> thanks for spotting this.  This was a typo, and was meant to read rotational signal. We did do a thorough analysis of the SAP flux and PLD detrended lightkurve and found similar rotation signals.
--> We inspected the SAP lightcurves.  Although they show ramps due to spacecraft systematics, they do not show any extra evidence of rotation signals that were removed by PDC.  Given that we have checked the PLD and SAP lightcurves yield consistent results to the PDCSAP lightcurves, we conclude that using the PDCSAP LC is appropriate in this analysis.  
-> We have added a sentence addressing the potential that these signals are potentially spurious and may be caused by spacecraft systematics. 
-> We have already state what the FAP are for these periods in the TESS data. 


I suspect it's not likely a coincidence that the WASP rotation period agrees perfectly with vsini assuming i=90, i.e. the orbit and spin are more likely to be aligned, and the 6-7 day signal is more likely not to be real: "Figure 5 shows a prominent peak at 14.2 days (Vrot = 3.58 km s−1) in the 2006/2007 season of data which matches the rotation period expected from the spectroscopic �� sin �� assuming a rotational inclination of 90 degrees." The final sentence of the paragraph "It is unclear whether the true rotation period is in the 5-7 or 14-17 day range" may be accurate given the lack of a quantitative comparison between the different rotation period estimates (e.g. via false-alarm probabilities, as was presented for the RV data). However, given the agreement between vsini and both of the WASP datasets, it may be more appropriate to discuss the a priori alignment probability, and/or the probability of such a coincidence if the system is in fact misaligned. Better yet, quantify the significance of the signals, and determine which period is better supported by the data. It is probably also worth pointing out here that the HARPS data appear to contain a significant signal at 12.9 days, which is closer to 14 days than 7 days. If there exist significant photometric signals sufficiently close to a significant RV signal, then there is probably a common origin, e.g. rotation.



-> We have added the false-alarm probability to Figure 5 and 6 to help quantify these signals.
-> We have added a discussion about the "a priori alignment probability" in the last paragraph. 
-> We have also moved our text discussing the pre-whitening of RVs here as an extra paragraph. Consequently, we have adjusted our text in Section 6.


Besides quantifying the significance of the signals from different datasets for comparison, it could also be worth employing other commonly used tools to measure rotational spot modulation: the autocorrelation function (ACF), gaussian processes (GPs) with an appropriate choice of kernel (e.g. quasi-periodic), or even phase dispersion minimization. This would strengthen the analysis and give the reader a better impression that speculation about a misaligned orbit is justified. Alternatively, weaker statements about (and less time spent discussing the possibility of) a misaligned orbit may be more appropriate, as a robust determination of the rotation period for this star may be difficult. 
--> We agree that weaker statements regarding the misalignment of the orbit are required here. To that end, we have removed our discussion regarding the misaligment and replaced it with a much weaker statement of the aligment. here we discusse the apriori aligment of the system and that the rotation period is more likely to be 14-17 days and aligned. 

The next paragraph is confusing: "We estimate a significant spin-orbit misalignment of almost ∼65◦ for a rotation signal between 14-17 days indicating the forma-tion of TOI-2447 b likely involved dynamical scattering or other orbit-tilting processes. A rotation signal between 5-7 days sug- gests an aligned system as expected from tidal migration." How is this consistent with your earlier statement that vsini in Table 1 (3.5 km/s) agrees perfectly with a rotation period of 14.5 days assuming i=90 degrees? Indeed, if I take your vsini (3.5 km/s) and stellar radius (1.006 Rsun) from Table 1, I get 14.5 days (assuming i=90 deg), so I can confirm that your earlier statement is these statements are is not. Alternatively, applying Equation 1 from Masuda & Winn 2020 gives me i=85.7 deg for a 14.5 d period, i.e. an aligned orbit.
--> Our apologies, we confused these two sets of numbers and that we instead should have stated that 14-17 day rotation  suggests an aligned system as expected from tidal migration, while we infer spin-orbit misalignment of almost ∼65◦ for a rotation signal between 5-7 days .
--> We have changed our discussion on this and moved it to the end.

Assuming the 2-sigma lower limit of your vsini measurement (2.3 km/s), I get an upper limit on the rotation period of 22 days. So, perhaps the simplest solution would be to present the various estimates of the rotation period from photometry, preferably along with quantification of their signal significance (or some other reliability metric), and conclude by saying that all of them are consistent with the upper limit on the rotation period from vsini. If in fact a strong case can be made that the signals at shorter periods are a) significant (i.e. not just noise), and b) not the result of issues pertaining to the input data, then discussion of the (mis)alignment of the system would be far more justified. On the other hand, if both sets of periods meet these criteria, then perhaps a deeper investigation of the data quality is needed, e.g. moonlight contamination (14.5 days is the first harmonic of the lunar cycle). In any case, without a more quantitative/careful/clear handling of the rotation period, it seems like a bit of a reach to discuss the alignment any further than a simple sentence, e.g. something like "more data are needed to constrain alignment via measurement of the rotation period or the R-M effect". 
--> We agree with what is suggested here. We have re-written the last paragraph to give more tentative statements about the alignemnt of the system, and commented on the Vsini upper limit and concluded that an RM measuremnt is needed, as suggested. We feel that this new conclusion to this section better reflects the quality of the measurements and what we can infer from the data. 
--> It is a good point to note that 14.5 is close to the half lunar cycle, which we know affects WASP data.  We therefore add a sentence of caution to the 2nd paragraph discussing WASP data. 
--> We have prefaced paragraph 1 with a clear statement that rotation rates can be difficult to determine for old/quite stars. 
--> We have also taken care to ensure the false-alarm probabilites have been reported for each period in section 4.2. 







Below are some minor issues that also need attention: 

Sec. 1 
-- 
small number of finite number of -> small number of 
--> Done.

Sec. 2 
-- 
we used a iterative algorithm -> we used an iterative algorithm
--> Done

one at the South African Astronomical Observatory (SAAO), South Africa, and another at the Observatorio del Roque de los Muchachos, La Palma - to be self-consistent, provide a more specific location for SAAO (Sutherland) as was done for the other observatory, instead of the country (which is already in the name) 
--> Changed South Africa to Sutherland.

However, significant systematic trends remain - remain after what? If you tried to detrend it, describe that, otherwise use a more appropriate wording.
-> We have added the text "Data from each observatory were detrended and aligned between different cameras and years using the TAMUZ algorithm \citep[][Cameron refers to the TAMUZ correction as SYSREM]{2006MNRAS.373..799C}.".

Are these systematics a problem because they are on the same timescale as transits, or are they longer-term trends that could be removed, e.g. with your iterative algorithm? 
-> These trends are sizable and on the same time scale as the transit signal; an iterative SG filter would be no good here.
-> We have changed the last sentence " However, significant systematic trends remain on the timescale of the transit width and these data are unsuitable for the search for single transits of additional planets.".

suggesting the presence transit timing variations -> suggesting the presence of transit timing variations 
--> Done.

Sec. 4 
-- 
capable of recovering photometric modulation attributed to stellar rotation -> 
capable of recovering photometric modulation due to stellar rotation 
-->Done

exceed time between -> exceed the time between 
--> Done

peak suggesting a rotation period of 17.1 days -> peak at 17.1 days 
peak suggesting a rotation period of 7.01 days -> peak at 7.01 days 
--> Done.

Figure 7 
-- 
Firstly, the caption uses inconsistent notation (black=solid vs black-dashed). Secondly, this information should be presented in a legend in the figure. Finally, including this figure without working harder to sort out the rotation period seems like a bit of a shame. If the data really can't distinguish the short/long period scenarios, is such a figure really adding value? If more information can be gleaned from the data, e.g. via more quantitative analysis, then this figure could more reasonably be presented in something close to its current form, i.e. with a solid black line representing the most likely scenario, and the dashed line representing the alternative for comparison. As it stands, that aspect of the figure is currently a bit misleading. 
--> We agree with the referees comments here. Ultimately, we decided to remove this figure and instead state more conservative comments regarding the rotation period and alignment of this system. See response to main concerns above. 


Sec. 5 
-- 
trail step -> trial step 
--> Changed

the semi-major axis was calculated by combining ��★ with ��★/a to calculate the semi- major axis, a - repetitious "the semi-major axis" and more importantly isn't this more precisely/reliably determined by using Kepler's 3rd law? 
--> We have adjusted this sentence "Furthermore, the semi-major axis, $a$, was calculated by combining $R_\star$ with $R_\star/a$."
--> Yes, this is determined through keplers 3rd law. We re-parametise this and calculate it through precisesly measuring the transit width, which in-turn depends on orbital period and eccentricity.


Sec. 6 
-- 
excluded with Sector 5 data -> excluded by Sector 5 data 
--> Done
NGTS data exclude some longer periods - what period ranges are excluded, at least approximately? 
--> Periods of 60-80 days are excluded for the most part with some gaps. Same for 100-120 days. Beyond that NGTS does not exclude any period.

Figure 11 
-- 
The caption states the signals "were fit and removed" but the details are not given here or in the text - were sinusoids fit and removed? Also, no mention of a possible origin for the 12.9 day signal is found here or in the text.
--> We have changed the sentence to include fitted and removed sinusoids "Signals above a false-alarm probability of 10\% were fit \textbf{with sinusoids} and removed until no peak existed above 10\%."
--> We have now referenced the 12.9 day signal in section 4.2 and discuss it in the context of additional planet signals. 
